Variable Rate Neural Compression for Sparse Detector Data

High-energy large-scale particle colliders generate data at extraordinary rates. Developing real-time high-throughput data compression algorithms to reduce data volume and meet the bandwidth requirement for storage has become increasingly critical. Deep learning is a promising technology that can address this challenging topic. At the newly constructed sPHENIX experiment at the Relativistic Heavy Ion Collider, a Time Projection Chamber (TPC) serves as the main tracking detector, which records three-dimensional particle trajectories in a volume of a gas-filled cylinder. In terms of occupancy, the resulting data flow can be very sparse reaching $10^{-3}$ for proton-proton collisions. Such sparsity presents a challenge to conventional learning-free lossy compression algorithms, such as SZ, ZFP, and MGARD. In contrast, emerging deep learning-based models, particularly those utilizing convolutional neural networks for compression, have outperformed these conventional methods in terms of compression ratios and reconstruction accuracy. However, research on the efficacy of these deep learning models in handling sparse datasets, like those produced in particle colliders, remains limited. Furthermore, most deep learning models do not adapt their processing speeds to data sparsity, which affects efficiency. To address this issue, we propose a novel approach for TPC data compression via key-point identification facilitated by sparse convolution. Our proposed algorithm, BCAE-VS, achieves a $75\%$ improvement in reconstruction accuracy with a $10\%$ increase in compression ratio over the previous state-of-the-art model. Additionally, BCAE-VS manages to achieve these results with a model size over two orders of magnitude smaller. Lastly, we have experimentally verified that as sparsity increases, so does the model's throughput.

==> src/method_data.tex <==
\subsection{TPC Data Preparation}
\label{subsec:dataet}

We demonstrate a simplified diagram of sPHENIX TPC in \autoref{fig:tpc_diagram}. The structure and working of a TPC can be simplified as follows. The TPC is a hollowed cylinder filled with a mixture of $75\%$ argon (\ce{Ar}), $20\%$ carbon tetrafluoride (\ce{CF4}), and $5\%$ isobutane gas. As a collision happens in the center of the TPC, it produce particles traversing the TPC's volume at nearly the speed of light. As a charged particle travels through the gas, it ionizes the gas atoms along its path, creating a trail of electrons. Due to the electric fields $E$, the electron cloud will drift towards either one of the two end plates (or readout plates). The positions and arrival times of the electrons are recorded by the sensors arranged in a circular grid on the readout plates. The density of the electron cloud allows us to distinguish different particle, e.g.~protons and pinons. A particle's trajectory will also be bend by an uniform magnetic field $B$ along the axial direction. This bending allows for the determination of the particles' momenta and charges based on the curvature of their trajectory.

\begin{figure}[ht]
    \centering
    \ifeditingfigure
        \tikzsetnextfilename{tpc_diagram}
        % \tikzexternaldisable
        \resizebox{.6\textwidth}{!}{\input{fig/tpc_diagram}}
    \else
        \resizebox{.6\textwidth}{!}{\includegraphics{fig/tpc_diagram.pdf}}
    \fi
    \caption{\textbf{A simplified diagram of Time-projection Chamber (TPC).}}
    \label{fig:tpc_diagram}
\end{figure}

The sPHENIX TPC has three layer groups: inner, middle, and outer. Each layer group produces a readout of a 3-dimensional (3D) array of ADC values. This array has $16$ layers along the radial direction and $249$ temporal sampling points along the axial direction on each side of the TPC. From the inside out, the three layer groups have an increasing number of sensors along the azimuthal direction. This number remains constant within a layer group. In this study, we will focus on the outer layer group of the TPC which has $2304$ sensors along the azimuthal direction. Each element in the readout array is called a \emph{voxel}. We demonstrate a full outer layer group readout in \autoref{fig:dataset}A (experiment $3060$, event $8$ in the test split of the \dsname dataset). 

\begin{figure}[ht]
    \centering
    \ifeditingfigure
        \tikzsetnextfilename{tpc_full_wedge_track}
        % \tikzexternaldisable
        \resizebox{\textwidth}{!}{\input{fig/tpc_full_wedge}}
    \else
        \resizebox{\textwidth}{!}{\includegraphics{fig/tpc_full_wedge_track.pdf}}
    \fi 
    \caption{The TPC outer layer group (Panel A) has dimensions $(16, 2304, 498)$ in the radial, azimuthal, and axial directions, respectively. This group is subdivided into $12$ sectors along the azimuthal direction and $2$ sides along the axial direction. Consequently, a TPC wedge (Panel B), representing one sector and one side of the full outer layer group, thus has dimensions $(16, 192, 249)$. From the zoom-in of an isolated trajectory (Panel C), we can see that a trajectory leaves a blob of signals on a layer and the location of the blobs vary smoothly. This means the location of the voxels belonging to one trajectory is highly correlated.}
    \label{fig:dataset}
\end{figure}

To match the subdivision of the TPC data assembly module in the readout chain, the data from a layer group is divided into $24$ equal-size non-overlapping section: $12$ along the azimuthal direction ($30$ degrees per section) and $2$ along the axial direction (separated by the transverse plane passing the collision point). We call one such section a \emph{TPC wedge}. In \autoref{fig:dataset}B, we zoom in on one of the wedges from the outer layer group. Each outer-layer wedge is a array of dimension $16$, $192$, and $249$ in radial, azimuthal, and axial directions, respectively. All ADC data from the same wedge will be transmitted to the same group of front-end electronics, after which a real-time lossy compression algorithm could be deployed. Therefore, TPC wedges are used as the direct input to the deep neural network compression algorithms.

To train a compression algorithm, we use the \dsname dataset\footnote{Zenodo linked:~\url{https://zenodo.org/records/10028587}}. This dataset contains $1310$ simulated events for central $\sqrt{s_{\mathrm{NN}}}=200$~GeV Au$+$Au collisions with 170~kHz pile-up collisions. The data were generated with the HIJING event generator~\cite{Wang:1991hta} and Geant4 Monte Carlo detector simulation package~\cite{Allison:2016lfl} integrated with the sPHENIX software framework~\cite{sPHENIX_Software}. 

The simulated TPC readout (ADC values) from these events are represented as $10$-bit unsigned integers $\in[0, 1023]$. To reduce unnecessary data transmission, a \emph{zero-suppression} algorithm has been applied. All ADC values below $64$ are suppressed to zero as most of them are noise. This zero-compression makes the TPC data sparse at about $10.8\%$ occupancy of non-zero values. We will call a voxel that has a non-zero ADC value a \emph{signal voxel}. A voxel with a $0$ ADC value will be called a \emph{non-signal voxel}. 

We divide the $1310$ total events into $1048$ events for training and $262$ for testing. Each event contains $24$ outer-layer wedges. Thus, the training partition contains $25152$ TPC outer-layer wedges, while the testing portion has $6288$. 

Finally, as trajectory locations must be interpolated from neighboring sensors using the ADC values, it is important to preserve the relative ADC ratio between the sensors. Hence, for this study, we work with \emph{log ADC values} (defined as $\log_2(\text{ADC} + 1)$) instead of the raw ADC values. A log ADC value is a float number $\in[0., 10.]$. Because of the zero-suppression at $64$, all nonzero log ADC values exceed $6$. The ground truth distribution of log ADC values is plotted in \autoref{fig:log_adc_distr}. Due to zero-suppression, the distribution of ADC is bimodal and extremely skewed. 

\begin{figure}[ht]
    \centering
    \ifeditingfigure
        \tikzsetnextfilename{log_adc_distr}
        % \tikzexternaldisable
        \input{fig/log_adc_distr}
    \else
        \includegraphics{fig/log_adc_distr.pdf}
    \fi 
    \caption{\textbf{Distribution of log ADC value.}}
    \label{fig:log_adc_distr}
\end{figure}

This distribution presents a significant challenge for neural network-based algorithms since neural network tends to work well when input data is distributed approximately normally~\cite{alanazi2020simulation,hashemi2019lhc}. In \autoref{subsec:bcae} we will show one approach to handle the discontinuity in the data distribution with a compression autoencoder equipped with two collaborating decoders. We will discuss the limitation of this approach and provide a better solution in \autoref{subsec:bcae_spoi} with sparse convolution. As a result, the sparsity of the data is no longer a obstacle to overcome but rather an advantage that we can leverage.  
